Structure and kinematics of a massive galaxy at z ~ 7

Observations of the rest-frame UV emission of high-redshift galaxies suggest that the early stages of galaxy formation involve disturbed structures. Imaging the cold interstellar medium can provide a unique view of the kinematics associated with the assembly of galaxies. In this paper, we analyzed the spatial distribution and kinematics of the cold ionized gas of the normal star-forming galaxy COS-2987030247 at z = 6.8076, based on new high-resolution observations of the [C II] 158um line emission obtained with the Atacama Large Millimeter/submillimeter Array. These observations allowed us to compare the spatial distribution and extension of the [C II] and rest-frame UV emission, model the [C II] line data-cube using 3DBarolo, and measure the [C II] luminosity and star formation rate (SFR) surface densities in the galaxy subregions. The system is found to be composed of a main central source, a fainter north extension, and candidate [C II] companions located 10-kpc away. We find similar rest-frame UV and [C II] spatial distributions, suggesting that the [C II] emission emerges from the star-forming regions. The agreement between the UV and [C II] surface brightness radial profiles rules out diffuse, extended [C II] emission in the main galaxy component. The [C II] velocity map reveals a velocity gradient in the north-south direction suggesting ordered motion, as commonly found in rotating-disk galaxies. But higher-resolution observations would be needed to rule out a compact merger scenario. Our model indicates a low average velocity dispersion, $\sigma$ < 30 km s$^{-1}$. This result implies a dispersion lower than the expected value from observations and semi-analytic models of high redshift galaxies. We argue that COS-2987030247 is a candidate rotating disk experiencing a short period of stability which will be possibly perturbed at later times by accreting sources.

==> trash.tex <==
## introduction



%The increase in the number of observations from [CII] emission in the last few years shows a significant fraction of galaxies with similar [CII] complex multi-clump structure, and indeed some objects have a good agreement with the stellar and cold neutral gaseous component. However, the majority of systems exhibit exotic behaviors such as a non-spatial correspondence between the brightest regions of [CII] and UV emission, and the presence of [CII] (UV) clumps with no UV ([CII]) counterparts. Regarding the centroids offset, Fujimoto et al. (2020) found a median offset of 0.15" which is similar to the astrometry offset of ALMA-HST data. But a significant fraction of systems reveals real physical differences (check sources from X X X X). It is still a open question what are the causing offsets but some explanations are proposed such as dust obscuration, stellar feedback and SSSSS. Furthermore, several objects display a more extended [CII] emission which indicates that the cold neutral gas can dominate the outer regions of early galaxies. Fujimoto et al. (2020) found in the ALPINE galaxies effective radius of [CII] from 2 to 3 times higher than the UV emission, with the ratio increasing with increasing stellar mass. The study also more extended radial profile ........ possible causes


